Affordances in Robotic Tasks -- A Survey

Affordances are key attributes of what must be perceived by an autonomous robotic agent in order to effectively interact with novel objects. Historically, the concept derives from the literature in psychology and cognitive science, where affordances are discussed in a way that makes it hard for the definition to be directly transferred to computational specifications useful for robots. This review article is focused specifically on robotics, so we discuss the related literature from this perspective. In this survey, we classify the literature and try to find common ground amongst different approaches with a view to application in robotics. We propose a categorisation based on the level of prior knowledge that is assumed to build the relationship among different affordance components that matter for a particular robotic task. We also identify areas for future improvement and discuss possible directions that are likely to be fruitful in terms of impact on robotics practice.

==> references <==
%intro
@article{bohg2017interactive,
  title={Interactive perception: Leveraging action in perception and perception in action},
  author={Bohg, Jeannette and Hausman, Karol and Sankaran, Bharath and Brock, Oliver and Kragic, Danica and Schaal, Stefan and Sukhatme, Gaurav S},
  journal={IEEE Transactions on Robotics},
  volume={33},
  number={6},
  pages={1273--1291},
  year={2017},
  publisher={IEEE}
}

@inproceedings{mcgrenere2000affordances,
  title={Affordances: Clarifying and evolving a concept},
  author={McGrenere, Joanna and Ho, Wayne},
  booktitle={Graphics interface},
  volume={2000},
  pages={179--186},
  year={2000}
}

@article{piaget1952origins,
  title={The origins of intelligence in children.},
  author={Piaget, Jean and Cook, Margaret Trans},
  year={1952},
  publisher={WW Norton \& Co}
}

@article{horton2012affordances,
  title={Affordances for robots: a brief survey},
  author={Horton, Thomas E and Chakraborty, Arpan and Amant, Robert St},
  journal={AVANT. Pismo Awangardy Filozoficzno-Naukowej},
  volume={2},
  pages={70--84},
  year={2012}
}

@article{jamone2018affordances,
  title={Affordances in psychology, neuroscience, and robotics: A survey},
  author={Jamone, Lorenzo and Ugur, Emre and Cangelosi, Angelo and Fadiga, Luciano and Bernardino, Alexandre and Piater, Justus and Santos-Victor, Jos{\'e}},
  journal={IEEE Transactions on Cognitive and Developmental Systems},
  volume={10},
  number={1},
  pages={4--25},
  year={2018},
  publisher={IEEE}
}

@article{Rosman2011,
title={Learning spatial relationships between objects},
  author={Rosman, Benjamin and Ramamoorthy, Subramanian},
  journal={The International Journal of Robotics Research},
  volume={30},
  number={11},
  pages={1328--1342},
  year={2011},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{min2016affordance,
  title={Affordance research in developmental robotics: a survey},
  author={Min, Huaqing and Yi, Chang’an and Luo, Ronghua and Zhu, Jinhui and Bi, Sheng},
  journal={IEEE Transactions on Cognitive and Developmental Systems},
  volume={8},
  number={4},
  pages={237--255},
  year={2016},
  publisher={IEEE}
}

@article{chemero2007gibsonian,
  title={Gibsonian affordances for roboticists},
  author={Chemero, Anthony and Turvey, Michael T},
  journal={Adaptive Behavior},
  volume={15},
  number={4},
  pages={473--480},
  year={2007},
  publisher={Sage Publications Sage UK: London, England}
}

@article{csahin2007afford,
  title={To afford or not to afford: A new formalization of affordances toward affordance-based robot control},
  author={{\c{S}}ahin, Erol and {\c{C}}akmak, Maya and Do{\u{g}}ar, Mehmet R and U{\u{g}}ur, Emre and {\"U}{\c{c}}oluk, G{\"o}kt{\"u}rk},
  journal={Adaptive Behavior},
  volume={15},
  number={4},
  pages={447--472},
  year={2007},
  publisher={Sage Publications Sage UK: London, England}
}

@article{symes2007visual,
  title={Visual object affordances: Object orientation},
  author={Symes, Ed and Ellis, Rob and Tucker, Mike},
  journal={Acta psychologica},
  volume={124},
  number={2},
  pages={238--255},
  year={2007},
  publisher={Elsevier}
}

@article{hartigan1979algorithm,
  title={Algorithm AS 136: A k-means clustering algorithm},
  author={Hartigan, John A and Wong, Manchek A},
  journal={Journal of the Royal Statistical Society. Series C (Applied Statistics)},
  volume={28},
  number={1},
  pages={100--108},
  year={1979},
  publisher={JSTOR}
}

@article{lafferty2001conditional,
  title={Conditional random fields: Probabilistic models for segmenting and labeling sequence data},
  author={Lafferty, John and McCallum, Andrew and Pereira, Fernando CN},
  year={2001}
}

@article{bishop2013model,
  title={Model-based machine learning},
  author={Bishop, Christopher M},
  journal={Phil. Trans. R. Soc. A},
  volume={371},
  number={1984},
  pages={20120222},
  year={2013},
  publisher={The Royal Society}
}

@article{trochim2001research,
  title={Research methods knowledge base},
  author={Trochim, William MK and Donnelly, James P},
  year={2001},
  publisher={Atomic Dog Pub.}
}

@inproceedings{jaakkola1999exploiting,
  title={Exploiting generative models in discriminative classifiers},
  author={Jaakkola, Tommi and Haussler, David},
  booktitle={Advances in neural information processing systems},
  pages={487--493},
  year={1999}
}

@inproceedings{taskar2002discriminative,
  title={Discriminative probabilistic models for relational data},
  author={Taskar, Ben and Abbeel, Pieter and Koller, Daphne},
  booktitle={Proceedings of the Eighteenth conference on Uncertainty in artificial intelligence},
  pages={485--492},
  year={2002},
  organization={Morgan Kaufmann Publishers Inc.}
}

@book{sutton1998introduction,
  title={Introduction to reinforcement learning},
  author={Sutton, Richard S and Barto, Andrew G},
  volume={135},
  year={1998},
  publisher={MIT press Cambridge}
}

@article{argall2009survey,
  title={A survey of robot learning from demonstration},
  author={Argall, Brenna D and Chernova, Sonia and Veloso, Manuela and Browning, Brett},
  journal={Robotics and autonomous systems},
  volume={57},
  number={5},
  pages={469--483},
  year={2009},
  publisher={Elsevier}
}

@inproceedings{gaver1991technology,
  title={Technology affordances},
  author={Gaver, William W},
  booktitle={Proceedings of the SIGCHI conference on Human factors in computing systems},
  pages={79--84},
  year={1991},
  organization={ACM}
}

@book{gibson2014ecological,
  title={The ecological approach to visual perception: classic edition},
  author={Gibson, James J},
  year={2014},
  publisher={Psychology Press}
}

@misc{norman1988psychology,
  title={The psychology of everyday things.(The design of everyday things)},
  author={Norman, Donald A},
  year={1988},
  publisher={Basic Books}
}

@article{bohg2014data,
  title={Data-driven grasp synthesis—a survey},
  author={Bohg, Jeannette and Morales, Antonio and Asfour, Tamim and Kragic, Danica},
  journal={IEEE Transactions on Robotics},
  volume={30},
  number={2},
  pages={289--309},
  year={2014},
  publisher={IEEE}
}

@article{turvey1992affordances,
  title={Affordances and prospective control: An outline of the ontology},
  author={Turvey, Michael T},
  journal={Ecological psychology},
  volume={4},
  number={3},
  pages={173--187},
  year={1992},
  publisher={Taylor \& Francis}
}
@article{stoffregen2003affordances,
  title={Affordances as properties of the animal-environment system},
  author={Stoffregen, Thomas A},
  journal={Ecological psychology},
  volume={15},
  number={2},
  pages={115--134},
  year={2003},
  publisher={Taylor \& Francis}
}

@article{chemero2003outline,
  title={An outline of a theory of affordances},
  author={Chemero, Anthony},
  journal={Ecological psychology},
  volume={15},
  number={2},
  pages={181--195},
  year={2003},
  publisher={Taylor \& Francis}
}

@inproceedings{steedman2002formalizing,
  title={Formalizing affordance},
  author={Steedman, Mark},
  booktitle={Proceedings of the Annual Meeting of the Cognitive Science Society},
  volume={24},
  number={24},
  year={2002}
}

@article{zech2017computational,
  title={Computational models of affordance in robotics: a taxonomy and systematic classification},
  author={Zech, Philipp and Haller, Simon and Lakani, Safoura Rezapour and Ridge, Barry and Ugur, Emre and Piater, Justus},
  journal={Adaptive Behavior},
  volume={25},
  number={5},
  pages={235--271},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}


% Model Base methods
@inproceedings{pandey2013affordance,
  title={Affordance graph: A framework to encode perspective taking and effort based affordances for day-to-day human-robot interaction},
  author={Pandey, Amit Kumar and Alami, Rachid},
  booktitle={Intelligent Robots and Systems (IROS), 2013 IEEE/RSJ International Conference on},
  pages={2180--2187},
  year={2013},
  organization={IEEE}
}

@article{fallon2015architecture,
  title={An architecture for online affordance-based perception and whole-body planning},
  author={Fallon, Maurice and Kuindersma, Scott and Karumanchi, Sisir and Antone, Matthew and Schneider, Toby and Dai, Hongkai and D'Arpino, Claudia P{\'e}rez and Deits, Robin and DiCicco, Matt and Fourie, Dehann and others},
  journal={Journal of Field Robotics},
  volume={32},
  number={2},
  pages={229--254},
  year={2015},
  publisher={Wiley Online Library}
}

@inproceedings{diana2013deformable,
  title={Deformable-medium affordances for interacting with multi-robot systems},
  author={Diana, Matteo and de la Croix, Jean-Pierre and Egerstedt, Magnus},
  booktitle={Intelligent Robots and Systems (IROS), 2013 IEEE/RSJ International Conference on},
  pages={5252--5257},
  year={2013},
  organization={IEEE}
}

@article{nielsen2007ecological,
  title={Ecological interfaces for improving mobile robot teleoperation},
  author={Nielsen, Curtis W and Goodrich, Michael A and Ricks, Robert W},
  journal={IEEE Transactions on Robotics},
  volume={23},
  number={5},
  pages={927--941},
  year={2007},
  publisher={IEEE}
}

@inproceedings{kim2014semantic,
  title={Semantic labeling of 3d point clouds with object affordance for robot manipulation},
  author={Kim, David Inkyu and Sukhatme, Gaurav S},
  booktitle={Robotics and Automation (ICRA), 2014 IEEE International Conference on},
  pages={5578--5584},
  year={2014},
  organization={Citeseer}
}

@inproceedings{aldoma2012supervised,
  title={Supervised learning of hidden and non-hidden 0-order affordances and detection in real scenes},
  author={Aldoma, Aitor and Tombari, Federico and Vincze, Markus},
  booktitle={Robotics and Automation (ICRA), 2012 IEEE International Conference on},
  pages={1732--1739},
  year={2012},
  organization={IEEE}
}


@article{Hart2015TheAT,
  title={The Affordance Template ROS package for robot task programming},
  author={Stephen Hart and Paul Dinh and Kimberly A. Hambuchen},
  journal={2015 IEEE International Conference on Robotics and Automation (ICRA)},
  year={2015},
  pages={6227-6234}
}

@article{castellini2011using,
  title={Using object affordances to improve object recognition},
  author={Castellini, Claudio and Tommasi, Tatiana and Noceti, Nicoletta and Odone, Francesca and Caputo, Barbara},
  journal={IEEE Transactions on Autonomous Mental Development},
  volume={3},
  number={3},
  pages={207--215},
  year={2011},
  publisher={IEEE}
}

@article{kjellstrom2011visual,
  title={Visual object-action recognition: Inferring object affordances from human demonstration},
  author={Kjellstr{\"o}m, Hedvig and Romero, Javier and Kragi{\'c}, Danica},
  journal={Computer Vision and Image Understanding},
  volume={115},
  number={1},
  pages={81--90},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{stark2008functional,
  title={Functional object class detection based on learned affordance cues},
  author={Stark, Michael and Lies, Philipp and Zillich, Michael and Wyatt, Jeremy and Schiele, Bernt},
  booktitle={International conference on computer vision systems},
  pages={435--444},
  year={2008},
  organization={Springer}
}

@inproceedings{cos2004using,
  title={Using a SOFM to learn object affordances},
  author={Cos-Aguilera, Ignasi and Hayes, G and Canamero, Lola},
  booktitle={Procs 5th Workshop of Physical Agents (WAF'04)},
  year={2004},
  organization={University of Edinburgh}
}

@article{katz2014perceiving,
  title={Perceiving, learning, and exploiting object affordances for autonomous pile manipulation},
  author={Katz, Dov and Venkatraman, Arun and Kazemi, Moslem and Bagnell, J Andrew and Stentz, Anthony},
  journal={Autonomous Robots},
  volume={37},
  number={4},
  pages={369--382},
  year={2014},
  publisher={Springer}
}
% Combined methods
@inproceedings{ugur2009affordance,
  title={Affordance learning from range data for multi-step planning},
  author={Ugur, Emre and Sahin, Erol and Oztop, Erhan},
  booktitle={Int. Conf. on Epigenetic Robotics},
  year={2009}
}

@article{do2017affordancenet,
  title={Affordancenet: An end-to-end deep learning approach for object affordance detection},
  author={Do, Thanh-Toan and Nguyen, Anh and Reid, Ian and Caldwell, Darwin G and Tsagarakis, Nikos G},
  journal={arXiv preprint arXiv:1709.07326},
  year={2017}
}

@inproceedings{koppula2016anticipatory,
  title={Anticipatory planning for human-robot teams},
  author={Koppula, Hema S and Jain, Ashesh and Saxena, Ashutosh},
  booktitle={Experimental Robotics},
  pages={453--470},
  year={2016},
  organization={Springer}
}
@inproceedings{ugur2007curiosity,
  title={Curiosity-driven learning of traversability affordance on a mobile robot},
  author={Ugur, Emre and Dogar, Mehmet R and Cakmak, Maya and Sahin, Erol},
  booktitle={Development and Learning, 2007. ICDL 2007. IEEE 6th International Conference},
  pages={13--18},
  year={2007},
  organization={IEEE}
}
@inproceedings{antunes2016human,
  title={From human instructions to robot actions: Formulation of goals, affordances and probabilistic planning},
  author={Antunes, Alexandre and Jamone, Lorenzo and Saponaro, Giovanni and Bernardino, Alexandre and Ventura, Rodrigo},
  booktitle={Robotics and Automation (ICRA), 2016 IEEE International Conference on},
  pages={5449--5454},
  year={2016},
  organization={IEEE}
}
@inproceedings{ugur2007learning,
  title={The learning and use of traversability affordance using range images on a mobile robot},
  author={Ugur, Emre and Dogar, Mehmet R and Cakmak, Maya and Sahin, Erol},
  booktitle={Robotics and Automation, 2007 IEEE International Conference},
  pages={1721--1726},
  year={2007},
  organization={IEEE}
}

@inproceedings{thomaz2009learning,
  title={Learning about objects with human teachers},
  author={Thomaz, Andrea L and Cakmak, Maya},
  booktitle={Proceedings of the 4th ACM/IEEE international conference on Human robot interaction},
  pages={15--22},
  year={2009},
  organization={ACM}
}

@inproceedings{barck2009learning,
  title={Learning grasping affordance using probabilistic and ontological approaches},
  author={Barck-Holst, Carl and Ralph, Maria and Holmar, Fredrik and Kragic, Danica},
  booktitle={Advanced Robotics, 2009. ICAR 2009. International Conference on},
  pages={1--6},
  year={2009},
  organization={IEEE}
}

@article{bohg2010learning,
  title={Learning grasping points with shape context},
  author={Bohg, Jeannette and Kragic, Danica},
  journal={Robotics and Autonomous Systems},
  volume={58},
  number={4},
  pages={362--377},
  year={2010},
  publisher={Elsevier}
}
@article{koppula2013learning,
  title={Learning human activities and object affordances from rgb-d videos},
  author={Koppula, Hema Swetha and Gupta, Rudhir and Saxena, Ashutosh},
  journal={The International Journal of Robotics Research},
  volume={32},
  number={8},
  pages={951--970},
  year={2013},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{montesano2008learning,
  title={Learning object affordances: from sensory--motor coordination to imitation},
  author={Montesano, Luis and Lopes, Manuel and Bernardino, Alexandre and Santos-Victor, Jos{\'e}},
  journal={IEEE Transactions on Robotics},
  volume={24},
  number={1},
  pages={15--26},
  year={2008},
  publisher={IEEE}
}

@inproceedings{fritz2006learning,
  title={Learning predictive features in affordance based robotic perception systems},
  author={Fritz, Gerald and Paletta, Lucas and Breithaupt, Ralph and Rome, Erich and Dorffner, Georg},
  booktitle={Intelligent Robots and Systems, 2006 IEEE/RSJ International Conference on},
  pages={3642--3647},
  year={2006},
  organization={IEEE}
}

@inproceedings{moldovan2012learning,
  title={Learning relational affordance models for robots in multi-object manipulation tasks},
  author={Moldovan, Bogdan and Moreno, Plinio and van Otterlo, Martijn and Santos-Victor, Jos{\'e} and De Raedt, Luc},
  booktitle={Robotics and Automation (ICRA), 2012 IEEE International Conference on},
  pages={4373--4378},
  year={2012},
  organization={IEEE}
}

@inproceedings{song2010learning,
  title={Learning task constraints for robot grasping using graphical models},
  author={Song, Dan and Huebner, Kai and Kyrki, Ville and Kragic, Danica},
  booktitle={Intelligent Robots and Systems (IROS), 2010 IEEE/RSJ International Conference on},
  pages={1579--1585},
  year={2010},
  organization={IEEE}
}

@article{bonaiuto2015learning,
  title={Learning to grasp and extract affordances: the Integrated Learning of Grasps and Affordances (ILGA) model},
  author={Bonaiuto, James and Arbib, Michael A},
  journal={Biological cybernetics},
  volume={109},
  number={6},
  pages={639--669},
  year={2015},
  publisher={Springer}
}

@article{sun2010learning,
  title={Learning visual object categories for robot affordance prediction},
  author={Sun, Jie and Moore, Joshua L and Bobick, Aaron and Rehg, James M},
  journal={The International Journal of Robotics Research},
  volume={29},
  number={2-3},
  pages={174--197},
  year={2010},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{montesano2007modeling,
  title={Modeling affordances using bayesian networks},
  author={Montesano, Luis and Lopes, Manuel and Bernardino, Alexandre and Santos-Victor, Jose},
  booktitle={Intelligent Robots and Systems, 2007. IROS 2007. IEEE/RSJ International Conference on},
  pages={4102--4107},
  year={2007},
  organization={IEEE}
}

@inproceedings{mar2015multi,
  title={Multi-model approach based on 3D functional features for tool affordance learning in robotics},
  author={Mar, Tanis and Tikhanoff, Vadim and Metta, Giorgio and Natale, Lorenzo},
  booktitle={Humanoid Robots (Humanoids), 2015 IEEE-RAS 15th International Conference on},
  pages={482--489},
  year={2015},
  organization={IEEE}
}

@article{kruger2011object,
  title={Object--action complexes: Grounded abstractions of sensory--motor processes},
  author={Kr{\"u}ger, Norbert and Geib, Christopher and Piater, Justus and Petrick, Ronald and Steedman, Mark and W{\"o}rg{\"o}tter, Florentin and Ude, Ale{\v{s}} and Asfour, Tamim and Kraft, Dirk and Omr{\v{c}}en, Damir and others},
  journal={Robotics and Autonomous Systems},
  volume={59},
  number={10},
  pages={740--757},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{nguyen2017object,
  title={Object-based affordances detection with convolutional neural networks and dense conditional random fields},
  author={Nguyen, Anh and Kanoulas, Dimitrios and Caldwell, Darwin G and Tsagarakis, Nikos G},
  booktitle={Intelligent Robots and Systems (IROS), 2017 IEEE/RSJ International Conference on},
  pages={5908--5915},
  year={2017},
  organization={IEEE}
}

@article{sun2014object,
  title={Object--object interaction affordance learning},
  author={Sun, Yu and Ren, Shaogang and Lin, Yun},
  journal={Robotics and Autonomous Systems},
  volume={62},
  number={4},
  pages={487--496},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{moldovan2014occluded,
  title={Occluded object search by relational affordances},
  author={Moldovan, Bogdan and De Raedt, Luc},
  booktitle={Robotics and Automation (ICRA), 2014 IEEE International Conference on},
  pages={169--174},
  year={2014},
  organization={IEEE}
}

@inproceedings{koppula2014physically,
  title={Physically grounded spatio-temporal object affordances},
  author={Koppula, Hema S and Saxena, Ashutosh},
  booktitle={European Conference on Computer Vision},
  pages={831--847},
  year={2014},
  organization={Springer}
}

@inproceedings{zhu2014reasoning,
  title={Reasoning about object affordances in a knowledge base representation},
  author={Zhu, Yuke and Fathi, Alireza and Fei-Fei, Li},
  booktitle={European conference on computer vision},
  pages={408--424},
  year={2014},
  organization={Springer}
}

@inproceedings{pieropan2014recognizing,
  title={Recognizing object affordances in terms of spatio-temporal object-object relationships},
  author={Pieropan, Alessandro and Ek, Carl Henrik and Kjellstr{\"o}m, Hedvig},
  booktitle={International Conference on Humanoid Robots, November 18-20th 2014, Madrid, Spain},
  pages={52--58},
  year={2014},
  organization={IEEE conference proceedings}
}

@inproceedings{wang2013robot,
  title={Robot learning and use of affordances in goal-directed tasks},
  author={Wang, Chang and Hindriks, Koen V and Babuska, Robert},
  booktitle={Intelligent Robots and Systems (IROS), 2013 IEEE/RSJ International Conference on},
  pages={2288--2294},
  year={2013},
  organization={IEEE}
}

@article{ugur2015staged,
  title={Staged development of robot skills: Behavior formation, affordance learning and imitation with motionese},
  author={Ugur, Emre and Nagai, Yukie and Sahin, Erol and Oztop, Erhan},
  journal={IEEE Transactions on Autonomous Mental Development},
  volume={7},
  number={2},
  pages={119--139},
  year={2015},
  publisher={IEEE}
}

@article{cruz2016training,
  title={Training agents with interactive reinforcement learning and contextual affordances},
  author={Cruz, Francisco and Magg, Sven and Weber, Cornelius and Wermter, Stefan},
  journal={IEEE Transactions on Cognitive and Developmental Systems},
  volume={8},
  number={4},
  pages={271--284},
  year={2016},
  publisher={IEEE}
}

@article{koppula2016anticipating,
  title={Anticipating human activities using object affordances for reactive robotic response},
  author={Koppula, Hema S and Saxena, Ashutosh},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={38},
  number={1},
  pages={14--29},
  year={2016},
  publisher={IEEE}
}

@inproceedings{hermans2011affordance,
  title={Affordance prediction via learned object attributes},
  author={Hermans, Tucker and Rehg, James M and Bobick, Aaron},
  booktitle={IEEE International Conference on Robotics and Automation (ICRA): Workshop on Semantic Perception, Mapping, and Exploration},
  pages={181--184},
  year={2011},
  organization={Citeseer}
}

@article{saxena2014robobrain,
  title={Robobrain: Large-scale knowledge engine for robots},
  author={Saxena, Ashutosh and Jain, Ashesh and Sener, Ozan and Jami, Aditya and Misra, Dipendra K and Koppula, Hema S},
  journal={arXiv preprint arXiv:1412.0691},
  year={2014}
}


% Exploratory Methods
@inproceedings{kroemer2012kernel,
  title={A kernel-based approach to direct action perception},
  author={Kroemer, Oliver and Ugur, Emre and Oztop, Erhan and Peters, Jan},
  booktitle={Robotics and Automation (ICRA), 2012 IEEE International Conference on},
  pages={2605--2610},
  year={2012},
  organization={IEEE}
}
@inproceedings{montesano2007affordances,
  title={Affordances, development and imitation},
  author={Montesano, Luis and Lopes, Manuel and Bernardino, Alexandre and Santos-Victor, Jose},
  booktitle={Development and Learning, 2007. ICDL 2007. IEEE 6th International Conference on},
  pages={270--275},
  year={2007},
  organization={IEEE}
}

@inproceedings{stoytchev2005toward,
  title={Behavior-grounded representation of tool affordances},
  author={Stoytchev, Alexander},
  booktitle={Proceedings of the 2005 ieee international conference on robotics and automation},
  pages={3060--3065},
  year={2005},
  organization={IEEE}
}

@inproceedings{hermans2013decoupling,
  title={Decoupling behavior, perception, and control for autonomous learning of affordances},
  author={Hermans, Tucker and Rehg, James M and Bobick, Aaron F},
  booktitle={Robotics and Automation (ICRA), 2013 IEEE International Conference on},
  pages={4989--4996},
  year={2013},
  organization={IEEE}
}

@inproceedings{bierbaum2009grasp,
  title={Grasp affordances from multi-fingered tactile exploration using dynamic potential fields},
  author={Bierbaum, Alexander and Rambow, Matthias and Asfour, Tamim and Dillmann, R{\"u}diger},
  booktitle={Humanoid Robots, 2009. Humanoids 2009. 9th IEEE-RAS International Conference on},
  pages={168--174},
  year={2009},
  organization={IEEE}
}

@inproceedings{tikhanoff2013exploring,
  title={Exploring affordances and tool use on the iCub},
  author={Tikhanoff, V and Pattacini, U and Natale, L and Metta, G},
  booktitle={Humanoid Robots (Humanoids), 2013 13th IEEE-RAS International Conference on},
  pages={130--137},
  year={2013},
  organization={IEEE}
}
@inproceedings{fitzpatrick2003learning,
  title={Learning about objects through action-initial steps towards artificial cognition},
  author={Fitzpatrick, Paul and Metta, Giorgio and Natale, Lorenzo and Rao, Sajit and Sandini, Giulio},
  booktitle={Robotics and Automation, 2003. Proceedings. ICRA'03. IEEE International Conference on},
  volume={3},
  pages={3140--3145},
  year={2003},
  organization={IEEE}
}

@inproceedings{de2006learning,
  title={Learning grasp affordances through human demonstration},
  author={de Granville, Charles and Southerland, Joshua and Fagg, Andrew H},
  booktitle={Proceedings of the International Conference on Development and Learning (ICDL’06)},
  year={2006}
}

@inproceedings{montesano2009learning,
  title={Learning grasping affordances from local visual descriptors},
  author={Montesano, Luis and Lopes, Manuel},
  booktitle={Development and Learning, 2009. ICDL 2009. IEEE 8th International Conference on},
  pages={1--6},
  year={2009},
  organization={IEEE}
}

@inproceedings{kraft2009learning,
  title={Learning objects and grasp affordances through autonomous exploration},
  author={Kraft, Dirk and Detry, Renaud and Pugeault, Nicolas and Ba{\c{s}}eski, Emre and Piater, Justus and Kr{\"u}ger, Norbert},
  booktitle={International Conference on Computer Vision Systems},
  pages={235--244},
  year={2009},
  organization={Springer}
}

@article{detry2011learning,
  title={Learning grasp affordance densities},
  author={Detry, Renaud and Kraft, Dirk and Kroemer, Oliver and Bodenhagen, Leon and Peters, Jan and Kr{\"u}ger, Norbert and Piater, Justus},
  journal={Paladyn, Journal of Behavioral Robotics},
  volume={2},
  number={1},
  pages={1--17},
  year={2011},
  publisher={De Gruyter Open}
}

@inproceedings{ivaldi2012perception,
  title={Perception and human interaction for developmental learning of objects and affordances},
  author={Ivaldi, Serena and Lyubova, Natalia and G{\'e}rardeaux-Viret, Damien and Droniou, Alain and Anzalone, Salvatore M and Chetouani, Mohamed and Filliat, David and Sigaud, Olivier},
  booktitle={Humanoid Robots (Humanoids), 2012 12th IEEE-RAS International Conference on},
  pages={248--254},
  year={2012},
  organization={IEEE}
}

@article{liu2018physical,
  title={Physical Primitive Decomposition},
  author={Liu, Zhijian and Freeman, William T and Tenenbaum, Joshua B and Wu, Jiajun},
  journal={arXiv preprint arXiv:1809.05070},
  year={2018}
}

@inproceedings{ugur2011unsupervised,
  title={Unsupervised learning of object affordances for planning in a mobile manipulation platform},
  author={Ugur, Emre and {\c{S}}ahin, Erol and Oztop, Erhan},
  booktitle={Robotics and Automation (ICRA), 2011 IEEE International Conference on},
  pages={4312--4317},
  year={2011},
  organization={IEEE}
}

% others
@article{garage2011turtlebot,
  title={Turtlebot},
  author={Garage, Willow},
  journal={Website: http://turtlebot. com/last visited},
  pages={11--25},
  year={2011}
}

@article{brunsdon1998geographically,
  title={Geographically weighted regression},
  author={Brunsdon, Chris and Fotheringham, Stewart and Charlton, Martin},
  journal={Journal of the Royal Statistical Society: Series D (The Statistician)},
  volume={47},
  number={3},
  pages={431--443},
  year={1998},
  publisher={Wiley Online Library}
}

@article{wold1987principal,
  title={Principal component analysis},
  author={Wold, Svante and Esbensen, Kim and Geladi, Paul},
  journal={Chemometrics and intelligent laboratory systems},
  volume={2},
  number={1-3},
  pages={37--52},
  year={1987},
  publisher={Elsevier}
}

@inproceedings{gonccalves2014learning,
  title={Learning intermediate object affordances: Towards the development of a tool concept},
  author={Gon{\c{c}}alves, Afonso and Abrantes, Jo{\~a}o and Saponaro, Giovanni and Jamone, Lorenzo and Bernardino, Alexandre},
  booktitle={4th International Conference on Development and Learning and on Epigenetic Robotics},
  pages={482--488},
  year={2014},
  organization={IEEE}
}

@inproceedings{myers2015affordance,
  title={Affordance detection of tool parts from geometric features},
  author={Myers, Austin and Teo, Ching L and Ferm{\"u}ller, Cornelia and Aloimonos, Yiannis},
  booktitle={2015 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={1374--1381},
  year={2015},
  organization={IEEE}
}

@inproceedings{jiang2013hallucinated,
  title={Hallucinated humans as the hidden context for labeling 3d scenes},
  author={Jiang, Yun and Koppula, Hema and Saxena, Ashutosh},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2993--3000},
  year={2013}
}

@article{asada2009cognitive,
  title={Cognitive developmental robotics: A survey},
  author={Asada, Minoru and Hosoda, Koh and Kuniyoshi, Yasuo and Ishiguro, Hiroshi and Inui, Toshio and Yoshikawa, Yuichiro and Ogino, Masaki and Yoshida, Chisato},
  journal={IEEE transactions on autonomous mental development},
  volume={1},
  number={1},
  pages={12--34},
  year={2009},
  publisher={IEEE}
}

@inproceedings{ardon2019learning,
  title={Learning Grasp Affordance Reasoning through Semantic Relations},
  author={Paola Ard{\'o}n and  {\`E}ric Pairet, and Ronald P. A. Petrick and Subramanian Ramamoorthy and Katrin S. Lohan},
  journal ={Robotics and Automation Letters (RA-L). To be presented at the International Conference on Intelligent Robots and Systems (IROS)},
  year = {2019},
 publisher={IEEE Robotics and Automation Letters},
 doi = {LRA.2019.2933815}
}

@article{huang2016recent,
  title={Recent data sets on object manipulation: A survey},
  author={Huang, Yongqiang and Bianchi, Matteo and Liarokapis, Minas and Sun, Yu},
  journal={Big data},
  volume={4},
  number={4},
  pages={197--216},
  year={2016},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}

%-------------------------------------
% part 2
@inproceedings{ruiz2018can,
  title={Where can i do this? Geometric Affordances from a Single Example with the Interaction Tensor},
  author={Ruiz, Eduardo and Mayol-Cuevas, Walterio},
  booktitle={f},
  pages={2192--2199},
  year={2018},
  organization={IEEE}
}

@inproceedings{ye2017can,
  title={What can i do around here? deep functional scene understanding for cognitive robots},
  author={Ye, Chengxi and Yang, Yezhou and Mao, Ren and Ferm{\"u}ller, Cornelia and Aloimonos, Yiannis},
  booktitle={2017 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={4604--4611},
  year={2017},
  organization={IEEE}
}

@article{chu2019learning,
  title={Learning affordance segmentation for real-world robotic manipulation via synthetic images},
  author={Chu, Fu-Jen and Xu, Ruinian and Vela, Patricio A},
  journal={IEEE Robotics and Automation Letters},
  volume={4},
  number={2},
  pages={1140--1147},
  year={2019},
  publisher={IEEE}
}

@inproceedings{kaiser2015validation,
  title={Validation of whole-body loco-manipulation affordances for pushability and liftability},
  author={Kaiser, Peter and Grotz, Markus and Aksoy, Eren E and Do, Martin and Vahrenkamp, Nikolaus and Asfour, Tamim},
  booktitle={2015 IEEE-RAS 15th International Conference on Humanoid Robots (Humanoids)},
  pages={920--927},
  year={2015},
  organization={IEEE}
}

@inproceedings{kaiser2016towards,
  title={Towards a hierarchy of loco-manipulation affordances},
  author={Kaiser, Peter and Aksoy, Eren E and Grotz, Markus and Asfour, Tamim},
  booktitle={2016 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={2839--2846},
  year={2016},
  organization={IEEE}
}

@inproceedings{ridge2010self,
  title={Self-supervised cross-modal online learning of basic object affordances for developmental robotic systems},
  author={Ridge, Barry and Sko{\v{c}}aj, Danijel and Leonardis, Ale{\v{s}}},
  booktitle={2010 IEEE International Conference on Robotics and Automation},
  pages={5047--5054},
  year={2010},
  organization={IEEE}
}

@inproceedings{bekiroglu2013predicting,
  title={Predicting slippage and learning manipulation affordances through gaussian process regression},
  author={Bekiroglu, Yasemin and Smith, Christian and Karayiannidis, Yiannis and Kragic, Danica and others},
  booktitle={2013 13th IEEE-RAS International Conference on Humanoid Robots (Humanoids)},
  pages={462--468},
  year={2013},
  organization={IEEE}
}

@inproceedings{song2013predicting,
  title={Predicting human intention in visual observations of hand/object interactions},
  author={Song, Dan and Kyriazis, Nikolaos and Oikonomidis, Iason and Papazov, Chavdar and Argyros, Antonis and Burschka, Darius and Kragic, Danica},
  booktitle={2013 IEEE International Conference on Robotics and Automation},
  pages={1608--1615},
  year={2013},
  organization={IEEE}
}

@article{song2015task,
  title={Task-based robot grasp planning using probabilistic inference},
  author={Song, Dan and Ek, Carl Henrik and Huebner, Kai and Kragic, Danica},
  journal={IEEE transactions on robotics},
  volume={31},
  number={3},
  pages={546--561},
  year={2015},
  publisher={IEEE}
}

@article{baleia2015exploiting,
  title={On exploiting haptic cues for self-supervised learning of depth-based robot navigation affordances},
  author={Baleia, Jos{\'e} and Santana, Pedro and Barata, Jos{\'e}},
  journal={Journal of Intelligent \& Robotic Systems},
  volume={80},
  number={3-4},
  pages={455--474},
  year={2015},
  publisher={Springer}
}

@inproceedings{gijsberts2010object,
  title={Object recognition using visuo-affordance maps},
  author={Gijsberts, Arjan and Tommasi, Tatiana and Metta, Giorgio and Caputo, Barbara},
  booktitle={2010 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={1572--1578},
  year={2010},
  organization={IEEE}
}

@inproceedings{nishide2009modeling,
  title={Modeling tool-body assimilation using second-order recurrent neural network},
  author={Nishide, Shun and Nakagawa, Tatsuhiro and Ogata, Tetsuya and Tani, Jun and Takahashi, Toru and Okuno, Hiroshi G},
  booktitle={2009 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={5376--5381},
  year={2009},
  organization={IEEE}
}

@article{aksoy2015model,
  title={Model-free incremental learning of the semantics of manipulation actions},
  author={Aksoy, Eren Erdal and Tamosiunaite, Minija and W{\"o}rg{\"o}tter, Florentin},
  journal={Robotics and Autonomous Systems},
  volume={71},
  pages={118--133},
  year={2015},
  publisher={Elsevier}
}

@article{song2015learning,
  title={Learning to detect visual grasp affordance},
  author={Song, Hyun Oh and Fritz, Mario and Goehring, Daniel and Darrell, Trevor},
  journal={IEEE Transactions on Automation Science and Engineering},
  volume={13},
  number={2},
  pages={798--809},
  year={2015},
  publisher={IEEE}
}

@article{aksoy2011learning,
  title={Learning the semantics of object--action relations by observation},
  author={Aksoy, Eren Erdal and Abramov, Alexey and D{\"o}rr, Johannes and Ning, Kejun and Dellen, Babette and W{\"o}rg{\"o}tter, Florentin},
  journal={The International Journal of Robotics Research},
  volume={30},
  number={10},
  pages={1229--1249},
  year={2011},
  publisher={Sage Publications Sage UK: London, England}
}

@inproceedings{erkan2010learning,
  title={Learning probabilistic discriminative models of grasp affordances under limited supervision},
  author={Erkan, Ay{\c{s}}e Naz and Kroemer, Oliver and Detry, Renaud and Altun, Yasemin and Piater, Justus and Peters, Jan},
  booktitle={2010 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={1586--1591},
  year={2010},
  organization={IEEE}
}

@inproceedings{chu2016learning,
  title={Learning object affordances by leveraging the combination of human-guidance and self-exploration},
  author={Chu, Vivian and Fitzgerald, Tesca and Thomaz, Andrea L},
  booktitle={2016 11th ACM/IEEE International Conference on Human-Robot Interaction (HRI)},
  pages={221--228},
  year={2016},
  organization={IEEE}
}

@inproceedings{hermans2013learning,
  title={Learning contact locations for pushing and orienting unknown objects},
  author={Hermans, Tucker and Li, Fuxin and Rehg, James M and Bobick, Aaron F},
  booktitle={2013 13th IEEE-RAS international conference on humanoid robots (humanoids)},
  pages={435--442},
  year={2013},
  organization={IEEE}
}

@inproceedings{dag2010learning,
  title={Learning affordances for categorizing objects and their properties},
  author={Dag, Nilgun and Atil, Ilkay and Kalkan, Sinan and Sahin, Erol},
  booktitle={2010 20th International Conference on Pattern Recognition},
  pages={3089--3092},
  year={2010},
  organization={IEEE}
}

@inproceedings{szedmak2014knowledge,
  title={Knowledge propagation and relation learning for predicting action effects},
  author={Szedmak, Sandor and Ugur, Emre and Piater, Justus},
  booktitle={2014 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={623--629},
  year={2014},
  organization={IEEE}
}

@inproceedings{kim2015interactive,
  title={Interactive affordance map building for a robotic task},
  author={Kim, David Inkyu and Sukhatme, Gaurav S},
  booktitle={2015 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4581--4586},
  year={2015},
  organization={IEEE}
}

@article{ugur2011goal,
  title={Goal emulation and planning in perceptual space using learned affordances},
  author={Ugur, Emre and Oztop, Erhan and Sahin, Erol},
  journal={Robotics and Autonomous Systems},
  volume={59},
  number={7-8},
  pages={580--595},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{dogar2007primitive,
  title={From primitive behaviors to goal-directed behavior using affordances},
  author={Dogar, Mehmet R and Cakmak, Maya and Ugur, Emre and Sahin, Erol},
  booktitle={2007 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={729--734},
  year={2007},
  organization={IEEE}
}

@article{lewis2005foot,
  title={Foot placement selection using non-geometric visual properties},
  author={Lewis, M Anthony and Lee, Hyo-Kyung and Patla, Aftab},
  journal={The International Journal of Robotics Research},
  volume={24},
  number={7},
  pages={553--561},
  year={2005},
  publisher={SAGE Publications}
}

@inproceedings{kaiser2014extracting,
  title={Extracting whole-body affordances from multimodal exploration},
  author={Kaiser, Peter and Gonzalez-Aguirre, David and Sch{\"u}ltje, Fabian and Borras, J{\'u}lia and Vahrenkamp, Nikolaus and Asfour, Tamim},
  booktitle={2014 IEEE-RAS International Conference on Humanoid Robots},
  pages={1036--1043},
  year={2014},
  organization={IEEE}
}

@inproceedings{song2011embodiment,
  title={Embodiment-specific representation of robot grasping using graphical models and latent-space discretization},
  author={Song, Dan and Ek, Carl Henrik and Huebner, Kai and Kragic, Danica},
  booktitle={2011 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={980--986},
  year={2011},
  organization={IEEE}
}

@inproceedings{chan2014determining,
  title={Determining proper grasp configurations for handovers through observation of object movement patterns and inter object interactions during usage},
  author={Chan, Wesley P and Kakiuchi, Yohei and Okada, Kei and Inaba, Masayuki},
  booktitle={2014 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={1355--1360},
  year={2014},
  organization={IEEE}
}

@inproceedings{dehban2016denoising,
  title={Denoising auto-encoders for learning of objects and tools affordances in continuous space},
  author={Dehban, Atabak and Jamone, Lorenzo and Kampff, Adam R and Santos-Victor, Jos{\'e}},
  booktitle={2016 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={4866--4871},
  year={2016},
  organization={IEEE}
}

@article{kostavelis2012collision,
  title={Collision risk assessment for autonomous robots by offline traversability learning},
  author={Kostavelis, Ioannis and Nalpantidis, Lazaros and Gasteratos, Antonios},
  journal={Robotics and Autonomous Systems},
  volume={60},
  number={11},
  pages={1367--1376},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{ugur2015bottom,
  title={Bottom-up learning of object categories, action effects and logical rules: From continuous manipulative exploration to symbolic planning},
  author={Ugur, Emre and Piater, Justus},
  booktitle={2015 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={2627--2633},
  year={2015},
  organization={IEEE}
}


@inproceedings{omrvcen2009autonomous,
  title={Autonomous acquisition of pushing actions to support object grasping with a humanoid robot},
  author={Omr{\v{c}}en, Damir and B{\"o}ge, Christian and Asfour, Tamim and Ude, Ale{\v{s}} and Dillmann, R{\"u}diger},
  booktitle={2009 9th IEEE-RAS International Conference on Humanoid Robots},
  pages={277--283},
  year={2009},
  organization={IEEE}
}

@inproceedings{varadarajan2012afrob,
  title={Afrob: The affordance network ontology for robots},
  author={Varadarajan, Karthik Mahesh and Vincze, Markus},
  booktitle={2012 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={1343--1350},
  year={2012},
  organization={IEEE}
}

@inproceedings{price2016affordance,
  title={Affordance-feasible planning with manipulator wrench spaces},
  author={Price, Andrew and Balakirsky, Stephen and Bobick, Aaron and Christensen, Henrik},
  booktitle={2016 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={3979--3986},
  year={2016},
  organization={IEEE}
}


@inproceedings{ridge2013action,
  title={Action-grounded push affordance bootstrapping of unknown objects},
  author={Ridge, Barry and Ude, Ales},
  booktitle={2013 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={2791--2798},
  year={2013},
  organization={IEEE}
}

@inproceedings{abelha2016model,
  title={A model-based approach to finding substitute tools in 3d vision data},
  author={Abelha, Paulo and Guerin, Frank and Schoeler, Markus},
  booktitle={2016 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={2471--2478},
  year={2016},
  organization={IEEE}
}

@inproceedings{sweeney2007model,
  title={A model of shared grasp affordances from demonstration},
  author={Sweeney, John D and Grupen, Rod},
  booktitle={2007 7th IEEE-RAS International Conference on Humanoid Robots},
  pages={27--35},
  year={2007},
  organization={IEEE}
}

@inproceedings{kroemer2011flexible,
  title={A flexible hybrid framework for modeling complex manipulation tasks},
  author={Kroemer, Oliver and Peters, Jan},
  booktitle={2011 IEEE International Conference on Robotics and Automation},
  pages={1856--1861},
  year={2011},
  organization={IEEE}
}

@article{cutsuridis2013cognitive,
  title={A cognitive control architecture for the perception--action cycle in robots and agents},
  author={Cutsuridis, Vassilis and Taylor, John G},
  journal={Cognitive Computation},
  volume={5},
  number={3},
  pages={383--395},
  year={2013},
  publisher={Springer}
}

@article{griffith2011behavior,
  title={A behavior-grounded approach to forming object categories: Separating containers from noncontainers},
  author={Griffith, Shane and Sinapov, Jivko and Sukhoy, Vladimir and Stoytchev, Alexander},
  journal={IEEE Transactions on Autonomous Mental Development},
  volume={4},
  number={1},
  pages={54--69},
  year={2011},
  publisher={IEEE}
}

@inproceedings{lopes2007affordance,
  title={Affordance-based imitation learning in robots},
  author={Lopes, Manuel and Melo, Francisco S and Montesano, Luis},
  booktitle={2007 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={1015--1021},
  year={2007},
  organization={IEEE}
}

==> sections/acknoledgments.tex <==
\section*{Acknowledgment}


The authors would like to thank...


==> sections/backup.tex <==
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \citet{lewis2005foot} The focus is to observe whether the robot’s foot placement changes when the affordance from the visual scene changes. Vision is important in interpreting non-geometric features of the environment that are important in supporting locomotion. They know the different scenarios and consequences of steping on the wrong patch.
        
        \citet{kostavelis2012collision} his work proposes a computationally efficient technique for the traversability estimation of the terrain, based on a machine learning classification method. ngstepextractsinformation-richfeaturesabout thecharacteristicsofthescene,whichareusedtotrainasupportvectormachine(SVM)separatingthe traversableandnon-traversables
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
         \citet{sweeney2007model} This paper presents a hierarchical, statistical topic  model  for  representing  the  grasp  preshapes  of  a set of objects. Observations provided by teleoperation are clustered into latent affordances shared among all objects. Each  affordance  defines a joint distribution over  position and  orientation  of  the  hand  relative  to  the  object  and conditioned on  visual  appearance.
         
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
        \citet{song2011embodiment,song2013predicting,song2015task} This paper presents a probabilistic frame-work for the representation and modeling of robot-grasping tasks. The framework consists of Gaussian mixture models for generic data discretization, and discrete Bayesian networks for encoding the probabilistic relations among various task-relevant variables, including  object  and  action  features  as  well  as  task  constraints. We evaluate the framework using a grasp database generated in a simulated environment including a human and two robot hand models. The generative modeling approach allows the prediction of grasping tasks given uncertain sensory data, as well as object and grasp selection in a task-oriented manner. a human tutor observes the 3-D configuration in a grasp simulator and provides labels of one or a set of afforded tasks from the task set (handover, pour-ing, tool use, dish washing, playing). The collected data are a set ofOG configurations instantiated with a set of{O, A, C} features together with the task labels T provided by human experts.  The approach allows for  generalization  over  task,  object,  and  action,  which  intro-duces a concept of embodiment-specific concept affordances. This allows us to perform and plan grasps across different em-bodiments  as  the  specific  affordances  are  independent  across embodiments.
        
        \citet{song2015task} they know objects-action-effects and what they are trying to learn are the grasping regions of the objects from multiple 2D images. SECTION II
        
        \citet{song2011embodiment} The contribution of this paper is to create a fully probabilistic framework for embodiment-specific representation of robot grasping tasks. We do this by integrating the BN approach from with the multi-variate discreitization model from. We demonstrate that the proposed framework successfully transfers task knowledge between different hands and provides the means for grasp planning and imitation in a goal-directed manner.
        
        \citet{dogar2007primitive} builds a set of goal-oriented behaviours based on primitive ones by linking the explored effects with previously seen environments. hree different behaviors achieved using the same three primitive behaviors and their learnedaffordance relations . In (a), the robot wanders around perceiving the traversability affordance of the object
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
         \citet{gijsberts2010object} htey create a visuo-map where a multi-modal classifier with real grasp information significantly boost object recognition. Knows all the the affordances.  The  affordances  considered  in  this  study  are  limited to  the  possible  types  of  grasp  that  can  reasonably  be  used with the particular object. We expect to see that these grasp affordances are highly discriminative for the object class and therefore improve object recognition significantly.perceiving known objects (i.e., the object identity is known to  the  agent). 2 In  the  second  variant  of  our  framework,  the  agent  would  always  have to  be  aware  of  the  object  identity  in  order  to  update  the  possible  grasp affordances for the objec
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
          %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \citet{price2016affordance} Our characterization revolves around the concept of a wrench space. agent-agent environment
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \cite{szedmak2014knowledge} they do knowledge propagation graph to try to build the relation betwee two objects by means of a missing edge.  their relative size. For example, while ‘inserted-in’ effect is generated when a small box is stacke d on a hollow cylinder, the ‘piled-up’ effect is observed when the box is larger than the opening on top of the cylinder.
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
           %------------------------------------------
        \textcolor{red}{add a sentence explaining the planning and fixed objects statement. (single affordance, single object and checking the effets to achieve an action)
        \citet{bekiroglu2013predicting} learns about slippage with different forces with a single object. in-hand to hand affordance
        \citet{omrvcen2009autonomous} Thereare   manysituationsin  which  anobject that needs  to  begraspedis notgraspable,but  could  begrasped if it wassituatedat  adifferentlocation. Byapplyingnon prehensile manipulationactions such  as  poking, theobject can  be moved to a  new  locationwithoutfirst  beinggrasped. We  propose  a learningprocessthatenables   the   robot   toacquirea general pushing  ruledescribingtherelationshipbetween thedirection of poke and  the observed  object  motion for a class of object.
         \citet{nishide2009modeling} they consider the tool as part of the body to push and reach red cylinder objects. In their approach they know already the relation of the affordance and they what to differianciate with which tool (T-shape, L-shap and I-shape) is better to achieve the task. }
         
         %----------------------------
    %----------------------------
    %----------------------------
    % \begin{table}[bt!]
    %     \centering
    %     \begin{tabular}{p{2.9cm}|p{1cm}|p{.5cm}|p{0.2mm} p{0.2mm} p{0.2mm}|p{0.2mm} p{0.2mm}}
    %     \hline
    %     \multirow{6}{*}{\textbf{Work}}&
    %     \multirow{6}{*}{\centering{\textbf{Robot}}}
    %     &\multirow{6}{*}{{\rotatebox[origin=c]{90}{\textbf{Application}}}}
    %     &\multicolumn{3}{c|}{\textbf{Perception}}
    %     &\multicolumn{2}{c}{\textbf{Actions}} \\
    %     \cline{4-8} & & &
    %     \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Visual}}}&
    %     \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Proprioception}}}&
    %     \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Tactile}}}&
    %     \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Primitive}}}&
    %     \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Complex}}} \\
    %     \hline
            
    %         \citet{kjellstrom2011visual} & N/A\textsuperscript{*} & M & \checkmark & & & \checkmark\\ \hline
    %         \mbox{\citet{diana2013deformable}} & Khepera III & N & \checkmark & & &  & \checkmark\\ \hline
    %         \mbox{\citet{pandey2013affordance}}  & PR2 & AP & \checkmark & & & &\checkmark \\ \hline
    %         \mbox{\citet{fallon2015architecture}}  & Atlas  & M & \checkmark &  & &  \checkmark &\checkmark\\ \hline
    %         \mbox{\citet{antunes2016human}} & iCub & M & \checkmark & & & \checkmark\\ \hline
    %         \mbox{\citet{thomaz2009learning}}  & Bioloid & M & \checkmark &  & & & \checkmark\\ \hline
    %         \citet{wang2013robot}  & NAO & AP & \checkmark & & & \checkmark \\ \hline
    %         \citet{cruz2016training}  & iCub & M & \checkmark & \checkmark & & \checkmark \\ \hline
    %         \mbox{\citet{do2017affordancenet}} & N/A  & AP && & & \checkmark & \checkmark \\ \hline
    %         \mbox{\citet{myers2015affordance}} & N/A  & AP && & & \checkmark & \checkmark \\ \hline
    %         \mbox{\citet{barck2009learning}} & Kuka \& Barret hand & M &  \checkmark & & & \checkmark\\ \hline
    %         \citet{sun2010learning} & PeopleBot and Rovio robot & N & \checkmark &  & &  & \checkmark \\ \hline
    %         \citet{sun2014object} & Fanuc \& Barret hand & M & \checkmark & \checkmark & & \checkmark & \checkmark \\ \hline
    %         \citet{moldovan2014occluded}  & N/A & AP & \checkmark & & & & \checkmark \\ \hline
    %         \citet{Hart2015TheAT} & Valkyrie \mbox{Robonaut2} & M & \checkmark & & & \checkmark \checkmark\\ \hline
    %         \citet{zhu2014reasoning} & N/A & AP & \checkmark & & & \checkmark &\checkmark \\ \hline
    %         \citet{saxena2014robobrain} & PR2 & M & \checkmark &  &  & & \checkmark\\ \hline
    %     \end{tabular}
    %     \raggedright N-Navigation; M-Manipulation and AP-Action Prediction.
    %     \raggedright \textsuperscript{*}Even though the application is for manipulation, no experiments are shown in a robot.
    %     \caption{Summary of works that have full \textit{a priori} knowledge of the affordance components relation for a task as prented in Section~\ref{sc:model}. \label{tb:known_data}}
    % \end{table}
    
    
    %----------------------------
%----------------------------
%----------------------------
    \begin{table}[t!]
        \centering
        \begin{tabular}{p{2.7cm}|p{1cm}|p{.5cm}|p{0.18mm} p{0.2mm} p{0.18mm}|p{0.2mm} p{0.2mm}}
        \hline
        \multirow{6}{*}{\textbf{Work}}&
        \multirow{6}{*}{\textbf{Robot}}
        &\multirow{6}{*}{{\rotatebox[origin=c]{90}{\textbf{Application}}}}
        &\multicolumn{3}{c|}{\textbf{Perception}}
        &\multicolumn{2}{c}{\textbf{Actions}}\\
        \cline{4-8} &&&
        \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Visual}}}&
        \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Proprioception}}}&
        \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Tactile}}}&
        \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Pimitive}}}&
        \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Complex}}} \\
        \hline
    
  
            \citet{cos2004using} & Khepera & N & \checkmark & & &  & \checkmark\\ \hline
            \citet{stark2008functional} & N/A\textsuperscript{*} & M & \checkmark & & & \checkmark & \checkmark\\ \hline
            \citet{castellini2011using} & N/A\textsuperscript{*} & M & \checkmark & & \checkmark & \checkmark\\ \hline
            \citet{aldoma2012supervised} & N/A & AP & \checkmark & & & & \checkmark\\ \hline
            \citet{kim2014semantic}  & PR2 & AP & \checkmark & & & \checkmark\\ \hline
            \citet{katz2014perceiving} & Barrett & M & \checkmark & \checkmark & & \checkmark\\ \hline
            \citet{gonccalves2014learning} & iCub & M & \checkmark & & & \checkmark\\ \hline
            \citet{fritz2006learning} & Kurt2 & N & \checkmark & & &  & \checkmark \\ \hline
            \citet{song2010learning}  & Barret hand & M & \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
            \mbox{\citet{ugur2009affordance}}  & Gifu Hand III  &  M & \checkmark & & & \checkmark \\ \hline
            \mbox{\citet{hermans2011affordance}}  & Pioneer 3 DX &  N  & \checkmark  & & & \checkmark\\ \hline
            \mbox{\citet{bohg2010learning}} & Armar head \& Kuka arm & M & \checkmark & & &\checkmark\\ \hline
            \citet{mar2015multi} & N/A & M & \checkmark &  & & \checkmark \\ \hline
            \citet{nguyen2017object} & WALK-MAN & AP & \checkmark &  & & \checkmark & \checkmark \\ \hline
            \mbox{\citet{moldovan2012learning}} & iCub & M & \checkmark & & & \checkmark \\ \hline
            \citet{tikhanoff2013exploring} & iCub & M & \checkmark & &  & \checkmark \\ \hline
            \mbox{\citet{de2006learning}} & P5 glove & M &  & & \checkmark & \checkmark\\ \hline
            \citet{kraft2009learning} & Staubli & M & \checkmark &   & \checkmark & \checkmark\\ \hline
            \citet{detry2011learning} & Barret hand & M &\checkmark & & \checkmark & \checkmark\\ \hline
            
        \end{tabular}
        \raggedright N-Navigation; M-Manipulation and AP-Action Prediction.
        \raggedright \textsuperscript{*}Even though the application is for manipulation, no experiments are shown in a robot.
        \caption{Summary of methods that have partial \textit{a priori} information on the affordance components relation to achieve a task as explained in Section~\ref{sc:combined}. \label{tb:combined_online_actions}}
  \end{table}
 
%----------------------------
%----------------------------
%----------------------------

\citet{abelha2016model} system connecting high level (i.e. a model) and low level (i.e. a point cloud) information, through a process of approximate matching that embodies some knowledge of what aspects of a tool are important for a particular task. They detect which part is the action part and which part is the handle. 

\citet{dag2010learning} achieved by deriving a condensed representation of the effects of actions (calledeffect prototypes in the paper), and investigating the relevance between perceptual fea-tures extracted from the objects and the actions that can be applied to them.Learning affordances for categorizing objects and their properties



\citet{griffith2011behavior} Framework used by the robot to l earn object categories. First, the robot interacts with the objects and observes t he outcomes that are produced. The ex-tracted auditory and visual features are u sed to learn perceptual outcome classes. These are used to form object categories, one for each behavior-modality com-bination. The categories are unifi ed using consensus clustering into a single cat-egory. Finally, a visual model is trained that can recognize the categories of novel objects. The dotted line is to show that the visual model could be used to guide and refi ne future interactions with objects. always shakes the objects to determine if they are container or not. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% to detect scenes
\citet{ye2017can} uses CNN to detect functional parts of objects in scene and tests on familiar scenes. 

\citet{aksoy2011learning} hereby, we encode the essential changes in a visual scenery in a condensed way such that a robot can recognize and learn a manipulation without prior object knowledge. To achieve this we continuously track image segments in the video and construct a dynamic graph sequence. Topological transitions of those graphs occur whenever a spatial relation between some segments has changed in a discontinuous way and these moments are stored in a transition matrix called the semantic event chain (SEC).

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \citet{ruiz2018can} with geometry they decide the affordance on familiar environements. object-object interaction
    
    \citet{chu2019learning} uses fast CNN to relate to familiar affordances. offers a dataset
    
    \citet{kaiser2014extracting} first part of the loco-manipulation affordances. Affordance hypotheses  are suggested  by rules that  incor-porate parameters of the primitives like orientation or extent. or  example,  a  planar  surface  that  is  sufficiently  large  and oriented  horizontally,  e.g.  a  table,  suggests  the  affordance support. 
    
    \citet{varadarajan2012afrob} affordances ontology based on superquadrics.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \citet{chan2014determining} it builds a KB based on observations on how a human hands over different objects. 
    
    \citet{ridge2013action} they dont know the objects but they know they need to push them and observe  the effects
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %navigation to go through
    \citet{baleia2015exploiting} This  article  presents  a  method  for  online learning  of  robot  navigation  affordances  from  spa-tiotemporally  correlated  haptic  and  depth  cues.  The method   allows   the   robot   to   incrementally   learn which  objects  present  in  the  environment  are  actu-ally traversable.
    
     \citet{kim2015interactive} A  PR2  robot  situated  in  a  simulated  warehouse  with disorganized  boxes  (left).  In  order  to  rearrange  boxes  at  desired positions,  the  robot  must  push  the  boxes.  But  some  boxes  cannot be pushed because they are blocked either by walls or other boxes. An affordance represents “pushability” in a certain direction. In this paper,  we  explore  how  to  learn  an  affordance  map  via  interactive manipulation in order to plan a rearrangement (right).
    
    %to grasp or push or reach
    \citet{erkan2010learning} grasp objects from the right position and orientation based on early cognitive vision (ECV) which uses descriptors of edges and such to generalise among objects. They use trial and error to collect data based on heuristics
    
    \citet{chu2016learning} We  compare  three  con-ditions:  (1)  learning  through  self-exploration,  (2)  learning  from supervised  examples  provided  by  10  na ̈ ıve  users,  and  (3)  self-exploration  biased  by  the  user  input.  Our  results  characterize the benefits of self and supervised affordance learning and show that a combined approach is the most efficient and successful
    
    \citet{hermans2013learning} the robot tries the push activity at many object locations based on geometry and evaluates the results to check if the object rolls or moves in straight line.
    
    \citet{dehban2016denoising} explores the environment and actively learns the affordances to reach the objects. 
    
    \citet{lopes2007affordance}  Prior to the experiments on imitation, the robot had already interacted with different objects and learned the affordance network for each of the 3 action primitives “Grasp”, “Tap” and “Touch”. The objects were classified according to the visual features “Color”, “Shape” and “Size” and the effects of each action in the objects were described in terms of “Velocity”, “Contact” and “Object-hand distance”. experiments with actions on known objects to find the effects. SECTION III
    
    %----------------------------
%----------------------------
%----------------------------
\begin{table}[b!]
    \centering
    \begin{tabular}{p{2.9cm}|p{1cm}|p{0.5cm}|p{0.2mm} p{0.2mm} p{0.2mm}|p{0.2mm} p{0.2mm}}
    \hline
    \multirow{6}{*}{\textbf{Work}}&
    \multirow{6}{*}{\textbf{Robot}}
    &\multirow{6}{*}{{\rotatebox[origin=c]{90}{\textbf{Application}}}}
    &\multicolumn{3}{c|}{\textbf{Perception}}
    &\multicolumn{2}{c}{\textbf{Actions}} \\
    \cline{4-8} & & &
    \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Visual}}}&
    \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Proprioception}}}&
    \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Tactile}}}&
    \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Primitive}}}&
    \parbox[c|]{0.3mm}{{\rotatebox[origin=c]{90}{Complex}}}\\
    \hline
         \citet{ugur2011unsupervised} & Kurt3D & N & \checkmark & & & \checkmark & \checkmark \\ \hline
         \citet{ugur2007curiosity} & Kurt3D  & M & \checkmark &  & &  & \checkmark\\ \hline
         \citet{ugur2015staged} & Motoman arm \& \mbox{Gifu hand}  & M & \checkmark & &\checkmark& & \checkmark \\ \hline
         \mbox{\citet{ugur2007learning}} & Kurt3D & M & \checkmark & &  & & \checkmark \\ \hline
         
         \mbox{\citet{montesano2007affordances}}  &  Baltazar & M & \checkmark & \checkmark &  & \checkmark\\ \hline
         \mbox{\citet{montesano2009learning}}& Baltazar & M & \checkmark &  &  & \checkmark\\ \hline
         \citet{montesano2007modeling} & Baltazar & M  & \checkmark &  & & \checkmark \\ \hline
         \mbox{\citet{montesano2008learning}} & Baltazar & M & \checkmark & &\checkmark  & \checkmark \\ \hline
         
         \citet{stoytchev2005toward} & CRS \& A251 & M & \checkmark & &  & \checkmark \\ \hline
         
         \mbox{\citet{hermans2013decoupling}} & PR2 & M & \checkmark & &  & \checkmark \\ \hline
         
         \citet{bierbaum2009grasp} & FRH-4 & M & \checkmark & & \checkmark & \checkmark \\ \hline
         \citet{fitzpatrick2003learning} & BabyBot \& Cog & M & \checkmark &  &  & \checkmark\\ \hline
         
         \citet{koppula2014physically} & N/A  & AP & \checkmark & & & & \checkmark \\ \hline
         \mbox{\citet{koppula2016anticipatory}} & PR2 & AP & \checkmark & &  &\checkmark & \checkmark \\ \hline
         \citet{koppula2013learning} & PR2 & AP & \checkmark &  & &\checkmark & \checkmark\\ \hline
         \citet{koppula2016anticipating} & PR2 & AP  &\checkmark &  &  & \checkmark & \checkmark\\ \hline
         \citet{jiang2013hallucinated} & PR2 & AP  &\checkmark &  &  & \checkmark & \checkmark\\ \hline
         \citet{ivaldi2012perception} & iCub & M &\checkmark & & &\checkmark \\ \hline
         
        \citet{liu2018physical} & N/A & AP & \checkmark & & & \checkmark & \checkmark \\ \hline
         
        \citet{bonaiuto2015learning} & N/A\textsuperscript{*}   & M & \checkmark & \checkmark & & \checkmark & \checkmark \\ \hline
          
          \mbox{\citet{pieropan2014recognizing}}  & N/A & AP & \checkmark & & &  &\checkmark \\ \hline
         
        \mbox{\citet{kroemer2012kernel}}  &  Allegro hand & M &\checkmark & \checkmark & & \checkmark & \checkmark\\ \hline
        
    \end{tabular}
    \raggedright N-Navigation; M-Manipulation and AP-Action Prediction.
     \raggedright \textsuperscript{*}Even though the application is for manipulation, no experiments are shown in a robot.
    \caption{Summary of methods that have no \textit{a priori} information on the affordance components relation to achieve a task, as summarised in Section~\ref{sc:exploratory}. \label{tb:exploratory}}
\end{table}
%----------------------------
%----------------------------
%----------------------------

\citet{ugur2011goal}we present the methods that enable the use of learnedaffordancestoaccomplishtaskswhichrequiresequential planning. 
    
    \citet{ugur2015bottom} The robot explores the environment using its action reper-toire, and encodes its observations in the form of continuou s world states and effects. While exploring the environment, the robot progressively acquires the ability to represent t he world with learned symbolic predicates, and to predict effe cts of its own actions based on learned logical rules. These predicates and rules are later used for symbolic planning
    
    
     \citet{kaiser2014extracting,kaiser2015validation,kaiser2016towards}, Use geometry primitives to extract the affordances for whole-body motion like upport, lean, grasp or hold and be performed in danger zone environments.. the extracted known primitives are assigned meaningful whole-body affordances. It is the continuation of the previous work. Now they propose a hierarchical affordances model built with primitive afforfances focussed on two types of grasping. Used for task planning. first part of the loco-manipulation affordances. Affordance hypotheses  are suggested  by rules that  incor-porate parameters of the primitives like orientation or extent. or  example,  a  planar  surface  that  is  sufficiently  large  and oriented  horizontally,  e.g.  a  table,  suggests  the  affordance support. They know about geometries with heuristics to check if it should grasp or navigate.
    %  \citeauthor{kaiser2016towards} & Armar III &\checkmark &\checkmark & & \checkmark & & &&& \checkmark & &&&\checkmark&\checkmark\\ \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \textcolor{red}{After interacting with the objects, the robot is ready to start the social phase of its development. In this section, we show how  to  use  affordances  in  this  context.  Imitation,  as  a  word used in everyday language, refers to many different behaviors}
    
       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \citet{ridge2013action} learns with heuristics. Although it is able to register only sliding and rolling.
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %both, exploration and lbd
    \citet{aksoy2015model} The SEC framework ana-14 lyzes the sequence of changes of thespatial relationsbetween the objects that 15 are being manipulated by a human or a robot. Consequently, SECs are invariant 16 to the particular objects used, the precise object poses observed, the actual tra-17 jectories followed, or the resulting interaction forces between objects.  
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    
    \centering
        \begin{tikzpicture}[timespan={},timeline width=25,scale=0.7,transform shape]
        
           %\timeline[custom interval=true]{1995-2007, 2008, 2009, 2010, 2011, 2012,2013, 2014, 2015, 2016, 2017, 2018, 2019}
        
        % % put here the phases
        % \begin{phases}
        % \initialphase{involvement degree=1.75cm,phase color=black}
        
        % \initialphase{involvement degree=1.75cm,phase color=black}
        
        % \tikzset{phase appearance/.append style={
        %   rectangle, 
        %   minimum width=\involvdegree,
        %   minimum height=3cm
        %  }
        % }
        % \phase{between year=2.5 and 4 in 0.5,phase color=green!80!black,involvement degree=7cm}
        
        % \phase{between year=10 and 11 in 0.5,phase color=green!80!black,involvement degree=1cm}
        
        % \end{phases}
        
        % % put here the milestones
        % \addmilestone{at=phase-0.90,direction=90:1cm,text={Based psychology formalisms},text options={above}}
        % %\addmilestone{at=phase-0.270,direction=270:1cm,text={Initial meeting},text options={below}}
        % \addmilestone{at=phase-1.270,direction=270:1cm,text={Based on the robot formalisms},text options={below}}
        % \addmilestone{at=phase-2.270,direction=270:1cm,text={Based on the robot formalism},text options={below}}
        % \end{tikzpicture}
        
        %\resizebox{16cm}{5cm}{
    %   \begin{tikzpicture}[timespan={},scale=0.7, transform shape]
    %         \timeline[custom interval=true]{\bfseries 1995-2007, \bfseries 2007,\bfseries 2008,\bfseries 2009,\bfseries 2010,\bfseries 2011,\bfseries 2012,\bfseries 2013,\bfseries 2014,\bfseries 2015, \bfseries 2016, \bfseries 2017, \bfseries 2018}
            
    % \begin{phases}
    
    %         %up to 2007
    %         \phase{between year=1 and 2 in 0,involvement degree=2.25cm}
            
    %         %from 2007-2011
    %         \phase{between year=2 and 3 in 0,involvement degree=2.25cm,phase color=blue!80!cyan}
            
    %         \phase{between week=3 and 4 in 0,involvement degree=2.25cm,phase color=blue!80!cyan}
            
    %         \phase{between week=4 and 5 in 0,involvement degree=2.25cm,phase color=blue!80!cyan}
    
    
    %         %A 2018
    %         \phase{between week=3 and 4 in 0.5,involvement degree=2.25cm,phase color=green!50!black}
    %         %C 2018
    %         \phase{between week=4 and 5 in -0.1,involvement degree=2.25cm,phase color=green!50!black}
    %         %R 2018
    %         \phase{between week=4 and 5 in 1.4,involvement degree=2.25cm,phase color=green!50!black}
    
    
    % \end{phases}
    % %2014
    %         \begin{scope}[every node/.append style={alias=mynode-1}]
    %         \addmilestone{at=phase-1.270,direction=270:1.5cm,text={Psycology based formalisms},text
    %         options={below}}
    %         \end{scope}
            
    %     %2016
    
    %         % \addmilestone{at=phase-2.90,direction=90:3.5cm,text={Announcement},text options={above}}
    %         \begin{scope}[every node/.append style={alias=mynode-2}]
    %          \addmilestone{}
    %          \end{scope}
    
    %         % \addmilestone{at=phase-3.90,direction=90:2.5cm,text={Clarification},text options={above}}
    %          \begin{scope}[every node/.append style={alias=mynode-3}]
    %          \addmilestone{}
    %          \end{scope}
    
    %         % \addmilestone{at=phase-4.90,direction=90:1.5cm,text={Results},text options={above}}
    %          \begin{scope}[every node/.append style={alias=mynode-4}]
    %          \addmilestone{}
    %         \end{scope}
    
    %     %2018
    
    %         \addmilestone{at=phase-5.90,direction=90:3.5cm,text={Announcement},text options={above}}
    %         \begin{scope}[every node/.append style={alias=mynode-7}]
    %         \addmilestone{at=phase-5.270,direction=270:1.5cm,text={Date},text options={below}}
    %         \end{scope}
    
    %         \addmilestone{at=phase-6.90,direction=90:2.5cm,text={Clarification},text options={above}}
    %         \begin{scope}[every node/.append style={alias=mynode-8}]
    %         \addmilestone{at=phase-6.270,direction=270:2.5cm,text={Date},text options={below}}
    %         \end{scope}
    
    %         \addmilestone{at=phase-7.90,direction=90:1.5cm,text={Results},text options={above}}
    %         \begin{scope}[every node/.append style={alias=mynode-9}]
    %         \addmilestone{at=phase-7.270,direction=270:3.5cm,text={Date},text options={below}}
    %         \end{scope}
    
    %         %%%%%
    %         \node[fit=(mynode-2)(mynode-3)(mynode-4)](f1){};
    %         \draw[decorate,decoration=brace,thick] (f1.south east) -- (f1.south west)
    %         node[midway,below]{something};
    %         \node[fit=(mynode-4)] (f2){};
    %         \draw[decorate,decoration=brace,thick] (f2.south east) -- (f2.south west)
    %         node[midway,below]{something else};
    %         \node[fit=(mynode-7) (mynode-8) (mynode-9)] (f3){};
    %         \draw[decorate,decoration=brace,thick] (f3.south east) -- (f3.south west)
    %         node[midway,below]{hibernate};
    \end{tikzpicture}
                  % }
